Self-Supervised Deep Learning for Model Correction in the Computational Crystallography Toolbox

The Computational Crystallography Toolbox (CCTBX) is open-source software that allows for processing of crystallographic data, including from serial femtosecond crystallography (SFX), for macromolecular structure determination. We aim to use the modules in CCTBX to determine the oxidation state of individual metal atoms in a macromolecule. Changes in oxidation state are reflected in small shifts of the atom's X-ray absorption edge. These energy shifts can be extracted from the diffraction images recorded in serial femtosecond crystallography, given knowledge of a forward physics model. However, as the diffraction changes only slightly due to the absorption edge shift, inaccuracies in the forward physics model make it extremely challenging to observe the oxidation state. In this work, we describe the potential impact of using self-supervised deep learning to correct the scientific model in CCTBX and provide uncertainty quantification. We provide code for forward model simulation and data analysis, built from CCTBX modules, at https://github.com/gigantocypris/SPREAD , which can be integrated with machine learning. We describe open questions in algorithm development to help spur advances through dialog between crystallographers and machine learning researchers. New methods could help elucidate charge transfer processes in many reactions, including key events in photosynthesis.

==> notes.tex <==
\section{todo}

- Scientific or industrial value of the simulator

- Scientific validity of the model behind the simulator (e.g., link to a peer-reviewed scientific paper)

- Potential impact of combining the simulator with machine learning (Highly encouraged but optional)

- Pointer to real-world data associated with the simulator (Highly encouraged but optional); ask Nick if we can make a dataset public


\section{notes}

	References in onboarding docs: https://docs.google.com/document/d/1Cq9Ss6bdU-yLEAFr7JQXFOOeKKMwacuT3eu4jhbcmow/edit

	What is the point of this paper?
	SPREAD problem: This problem is truly a needle in a haystack
	This is a difficult problem as it requires an accurate forward model
	To solve the problem of SPREAD, the physical model must be refined with the collected data
	The purpose of this paper is to spur further conversation between crystallographers and machine learning practitioners to create data-driven algorithms to solve for the electronic state of individual atoms in chemical reactions
	
	Simulation paper made assumptions that may not hold in practice
	Forward model refinement may allow the additional benefit of being able to use more data, rather than filtering it out for not fitting well with the forward model
	These are the algorithmic advances/open questions that need to be solved
	
\section{dxtbx}

The Diffraction Experiment Toolbox dxtbx (Parkhurst et al., 2014[Parkhurst, J. M., Brewster, A. S., Fuentes-Montero, L., Waterman, D. G., Hattne, J., Ashton, A. W., Echols, N., Evans, G., Sauter, N. K. & Winter, G. (2014). J. Appl. Cryst. 47, 1459-1465.])

\section{Diffraction Integration for Advanced Light Sources (DIALS)}

Evans (2013)
scaling: variations in the incident-beam intensity, the volume of the crystal illuminated, absorption in the primary or secondary beam and average radiation damage

Notes from Winter (2017)
spot finding, indexing, refinement and integration
x-ray crystallography to find the atomic structure of biological macromolecules
created in response to larger numbers of smaller samples used in crystallography
open-source package
works with rotation data sets and still-shot diffraction data
DIALS is built upon the cctbx library

dxtbx to create the following objects: beam, goniometer, detector, source, crystal
find spots, then index them and update the crystal object
refine all the parameters of the objects using knowledge of the centroids of the spots
integrate the spots, and output the final Miller index (location in Fourier space, this is an integer index b/c only discrete spots in Fourier space), scale factor

2 major data structures: reflection table (pandas-like) list of all the spots (with spot integrated intensity, and Miller index, per reflection scale (e.g. more absorption of photos at an angle)
experiment list encodes the experimental geometry and crystal properties (unit cell parameters, crystal orientation, crystal mosaicity (number of domains and mis-orientation spread))
Each experiment has exactly one beam, detector and crystal model, with an optional goniometer and scan model; an experiment list is a collection of these

indexing goal: find the UB matrix from the centroids and geometry
from one still image: map the spots to reciprocal space and find the unit cell and orientation. unit cell is shared over all still shots, orientation is found per shot. use orientation to assign Miller index to each spot

can find multiple crystals from a still shot

Can refine geometry and orientation/unit cell/miller index separately and iteratively
refinement aims to minimize the different in the observed and predicted spot centroids

integration is next, attempt to remove the effect of the background around the spot and in the spot
shoebox: contains the peak pixels and a substantial border of background pixels surrounding the peak

bandedge is the K absorption edge

Notes on Mendez (2020)
serial femtosecond crystallography (SFX)
averaging integrated values over many measurements
A physical model describing all observed pixels
synthetic example where the anomalous difference signal is stable
mosaicity is the mosaic domain size and the mosaic rotational spread
partiality of each spot: per-reflection scale factor that accounts for Ewald offset

For the work presented in this paper, determination of optimal structure factors |Fh|, given the data, occurred in a single step, guided by a likelihood target function dependent on crystal orientations, unit cells, scale factors, mosaic parameters, photon spectra and, importantly, a starting list of structure factors provided by conventional data processing.

structure factor amplitudes and per-shot scale factors both directly increase the intensities of spots; however, in the global treatment, other shots measuring the same reflections constrain the structure factors.

total number of mosaic domains gives an overall scale factor
B is the diagonal matrix of unit cell parameters a,b,c
U is the 3x3 rotational matrix


Sauter (2015)
"While cctbx.xfel can fortunately calibrate sensor positions to about 0.1-pixel accuracy, it is found that even a 0.5-pixel miscalibration noticeably degrades the integrated data, and that this is felt most acutely for the highest-resolution data"
Have to make assumptions about the mosaic structure of the crystal
Problem of partiality

Pointer to data: A tutorial for processing the thermolysin data is presented at https://cci.lbl.gov/xfel .
Thermolysin diffraction patterns were reprocessed from a previously described data set (Hattne et al., 2014[Hattne, J. et al. (2014). Nat. Methods, 11, 545-548.]) that is publicly archived at the Coherent X-ray Imaging Data Bank (https://cxidb.org ), accession ID 23. 

Pointer to another dataset:
Simulated still-shot diffraction patterns from photosystem I (PSI) were obtained from James Holton (LBNL), and are available at https://bl831a.als.lbl.gov/example_data_sets/Illuin/LCLS . The 20000-image simulated dataset was created with the program fastBragg as described (Kirian et al., 2010[Kirian, R. A., Wang, X., Weierstall, U., Schmidt, K. E., Spence, J. C. H., Hunter, M., Fromme, P., White, T., Chapman, H. N. & Holton, J. (2010). Opt. Express, 18, 5713-5723.], 2011[Kirian, R. A., White, T. A., Holton, J. M., Chapman, H. N., Fromme, P., Barty, A., Lomb, L., Aquila, A., Maia, F. R. N. C., Martin, A. V., Fromme, R., Wang, X., Hunter, M. S., Schmidt, K. E. & Spence, J. C. H. (2011). Acta Cryst. A67, 131-140.]), utilizing modeled structure factors from Protein Data Bank entry 1jb0 .

each mosaic block can have a different unit cell!
need to produce a unit cell distribution for each crystal
for every spot, need scale factor to account for partiality


Brewster (2018)
``Diffraction modeling is an exercise in determining the experimental parameters, such as incident beam wavelength, crystal unit cell and orientation, and detector geometry, that are most consistent with the observed positions of Bragg spots.''


Hattne (2014)
cctbx.xfel
Each mosaic domain has a different unit cell
"Although SFX is presently a challenging technique, its potential payoff in terms of enabling specialized structural and dynamical studies of macromolecules is enormous."

Sauter (2014)
anomalous difference electron density
crystal orientation is not uniquely defined
Rotating around z axis moves the position of the Bragg peaks
Rotating around the x and y axis moves the spots in and out of the diffracting condition, can change the partiality

Photon Dynamics in Photosystem II as an Example Application:

Kern, J., Chatterjee, R., Young, I. D., Fuller, F. D., Lassalle, L., Ibrahim, M., Gul, S., Fransson, T., Brewster, A. S., Alonso-Mori, R., Hussein, R., Zhang, M., Douthit, L., de Lichtenberg, C., Cheah, M. H., Shevela, D., Wersig, J., Seuffert, I., Sokaras, D., Pastor, E., Weninger, C., Kroll, T., Sierra, R. G., Aller, P., Butryn, A., Orville, A. M., Liang, M., Batyuk, A., Koglin, J. E., Carbajo, S., Boutet, S., Moriarty, N. W., Holton, J. M., Dobbek, H., Adams, P. D., Bergmann, U., Sauter, N. K., Zouni, A., Messinger, J., Yano, J. \& Yachandra, V. K. (2018). Nature, 563, 421–425. 

Ibrahim, M., Fransson, T., Chatterjee, R., Cheah, M. H., Hussein, R., Lassalle, L., Sutherlin, K. D., Young, I. D., Fuller, F. D., Gul, S., Kim, I. S., Simon, P. S., de Lichtenberg, C., Chernev, P., Bogacz, I., Pham, C. C., Orville, A. M., Saichek, N., Northen, T., Batyuk, A., Carbajo, S., Alonso-Mori, R., Tono, K., Owada, S., Bhowmick, A., Bolotovsky, R., Mendez, D., Moriarty, N. W., Holton, J. M., Dobbek, H., Brewster, A. S., Adams, P. D., Sauter, N. K., Bergmann, U., Zouni, A., Messinger, J., Kern, J., Yachandra, V. K. \& Yano, J. (2020). Proc. Natl Acad. Sci. USA, 117, 12624–12635. 

Iris Young, Nature paper

https://www.nature.com/articles/s41586-023-06038-z

``Ultimately, our interest lies in single-electron transfers at the four Mn positions of the PSII catalytic cofactor. Spatially resolving the K absorption edge individually for each Mn center has the potential to elucidate the electronic environment of each Mn atom (Sauter et al., 2020[Sauter, N. K., Kern, J., Yano, J. \& Holton, J. M. (2020). Acta Cryst. D76, 176-192.])''


Sauter (2015)
"While cctbx.xfel can fortunately calibrate sensor positions to about 0.1-pixel accuracy, it is found that even a 0.5-pixel miscalibration noticeably degrades the integrated data, and that this is felt most acutely for the highest-resolution data"
Have to make assumptions about the mosaic structure of the crystal
Problem of partiality

Pointer to data: A tutorial for processing the thermolysin data is presented at https://cci.lbl.gov/xfel .
Thermolysin diffraction patterns were reprocessed from a previously described data set (Hattne et al., 2014[Hattne, J. et al. (2014). Nat. Methods, 11, 545-548.]) that is publicly archived at the Coherent X-ray Imaging Data Bank (\url{https://cxidb.org} ), accession ID 23. 

Pointer to another dataset:
Simulated still-shot diffraction patterns from photosystem I (PSI) were obtained from James Holton (LBNL), and are available at \url{https://bl831a.als.lbl.gov/example_data_sets/Illuin/LCLS} . The 20000-image simulated dataset was created with the program fastBragg as described (Kirian et al., 2010)

%[Kirian, R. A., Wang, X., Weierstall, U., Schmidt, K. E., Spence, J. C. H., Hunter, M., Fromme, P., White, T., Chapman, H. N. & Holton, J. (2010). Opt. Express, 18, 5713-5723.], 2011[Kirian, R. A., White, T. A., Holton, J. M., Chapman, H. N., Fromme, P., Barty, A., Lomb, L., Aquila, A., Maia, F. R. N. C., Martin, A. V., Fromme, R., Wang, X., Hunter, M. S., Schmidt, K. E. & Spence, J. C. H. (2011). Acta Cryst. A67, 131-140.]), utilizing modeled structure factors from Protein Data Bank entry 1jb0 .

\section{Datasets}

Are the datasets publicly available?
Simulated dataset/experimental dataset

Sauter (2015)

Pointer to data: A tutorial for processing the thermolysin data is presented at https://cci.lbl.gov/xfel .
Thermolysin diffraction patterns were reprocessed from a previously described data set (Hattne et al., 2014[Hattne, J. et al. (2014). Nat. Methods, 11, 545-548.]) that is publicly archived at the Coherent X-ray Imaging Data Bank (\url{https://cxidb.org} ), accession ID 23. 

Pointer to another dataset:
Simulated still-shot diffraction patterns from photosystem I (PSI) were obtained from James Holton (LBNL), and are available at \url{https://bl831a.als.lbl.gov/example_data_sets/Illuin/LCLS} . The 20000-image simulated dataset was created with the program fastBragg as described (Kirian et al., 2010)

[Kirian, R. A., Wang, X., Weierstall, U., Schmidt, K. E., Spence, J. C. H., Hunter, M., Fromme, P., White, T., Chapman, H. N. & Holton, J. (2010). Opt. Express, 18, 5713-5723.], 2011[Kirian, R. A., White, T. A., Holton, J. M., Chapman, H. N., Fromme, P., Barty, A., Lomb, L., Aquila, A., Maia, F. R. N. C., Martin, A. V., Fromme, R., Wang, X., Hunter, M. S., Schmidt, K. E. & Spence, J. C. H. (2011). Acta Cryst. A67, 131-140.]), utilizing modeled structure factors from Protein Data Bank entry 1jb0 .

\section{notes}
Sauter (2014)
anomalous difference electron density
crystal orientation is not uniquely defined
Rotating around z axis moves the position of the Bragg peaks
Rotating around the x and y axis moves the spots in and out of the diffracting condition, can change the partiality

\subsection{Shoebox Generation}



Mendoza (2022) and Olsen (2022) use the P-VAE for computed tomography and Fourier ptychographic microscopy, respectively. Sparse measurements are assumed to be over a dataset of similar sources. In solving for the anomalous structure factors in serial femtosecond crystallography, we face a similar problem with some important differences. We have many images of crystals, and each crystal is of the same underlying material and structure factors, but has differences in the size, mosaicity, orientation, and unit cell. Our objective is to reconstruct the anomalous structure factors, which are common to all examples of the dataset. Like Mendoza (2022) and Olsen (2022), we reconstruct all the sources (i.e. crystals) of the dataset (in this case, per-source parameters such as the unit cell and orientation), but unlike in the previous work, this serves only in the larger mission to reconstruct the anomalous structure factors.

Warm start might be similar to some of the other loss functions in the Takeishi paper



each mosaic block can have a different unit cell!
need to produce a unit cell distribution for each crystal
for every spot, need scale factor to account for partiality

Each mosaic domain has a different unit cell [REF: Hattne (2014)]

We aim to create the underlying model that generates shoeboxes that are indistinguishable from our experimentally measured shoeboxes
Minimize divergence from the modeled distribution

Underlying latent parameters:
Shoebox level: Miller index, partiality (Ewald offset), diffraction spot scale
Image level: orientation, unit cell, mosaicity, incident spectrum, total flux
Dataset level: atom positions in the unit cell. $B_m$, non-anomalous scattering factor of the atom, anomalous scattering factor of the atom

Figure, pg. 17

The proposed framework is inspired by variational autoencoders. The basic idea is to optimize the neural network such that it outputs generated shoeboxes that come from the same underlying distribution as the actual shoeboxes. More precisely, we train this structure so that the actual shoeboxes are generated with high probability (maximize P(actual shoeboxes)).

For efficient optimization, the variational autoencoder includes an “encoder” (with the above serving as the “decoder”). Generally, the encoder is another neural network. Here, we directly optimize the latent variables by finding a mean and variance for each latent variable, per shoebox. The latent variables may be global (e.g. the structure factors), per image (e.g. detector position), or per shoebox (e.g. tilt plane coefficients). We formulate as a conditional autoencoder; the variables conditioned on are the input photon spectrum and the pixel coordinates of the shoebox (both are assumed to be known exactly).

The quantities for each level of the hierarchy are enumerated below. The distribution Q(x), where x is the latent space variable and Q is the approximation to the prior distribution, will be specified as a Gaussian with a mean and variance. There will be a latent space variable for each quantity of interest in the forward model. The mean and variance for each latent space variable will be consistent across the hierarchical level (e.g. the same for all shoeboxes in an image). The shoeboxes, as in the state-of-the-art, will be extracted using DIALS. 

The forward model may have inaccuracies that we don’t know about. Thus, at all levels (global, image, shoebox), we can optimize a set of latent variables to represent the related unknown quantities (the same as in the above image under “For each quantity.” After the “Forward Model” (bottom of the above image),  we can insert a neural network which takes in these quantities and completes further processing before outputting the predicted shoebox distribution (see below). The figure of merit to optimize the variational autoencoder will include 3 metrics: the KL divergence of the approximation with the latent variable priors, the likelihood of the data, and the KL divergence between the unmodified forward model result and the modified forward model result.

Optimizing Eqn. XX to maximize the probability of generating the experimentally measured shoeboxes is computationally difficult as given a shoebox, as most random samples will give a probability of 0 to the shoebox. We solve this problem by modifying the shoebox generator into a physics-informed variational autoencoder (P-VAE)

Encoder Input Quantities for every shoebox:

Dataset level:
N/A

Full detector image:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Overall scale factor
Measured spectrum
Orientation from DIALS
Mosaicity parameters (shape of domains, size of domains)
Unit Cell
Optimizable input variable


Quadrant level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


Sensor array level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


ASIC level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


Shoebox:
Shoebox pixels
Background mask from DIALS
Foreground mask from DIALS
Background tilt plane coefficients from \textsc{nanoBragg}
Pixel positions
Optimizable input variable

Decoder Output Quantities:

calculated from pixel and detector positions --> Miller index from \textsc{DIALS}

Dataset level:
Anomalous corrections to scattering factors of metal atoms near the \textit{K} edge as a function of wavelength, delta from Henke tables value
atom positions in the unit cell of the metal atoms near the K-edge --> delta from known values
$B_m$ --> fixed
non-anomalous structure factor of the atom --> delta from the merging final values/nanoBragg refinement
Arbitrary parameters 
 
Full detector image:
Total flux of incident photon spectrum
Base detector position
Crystal orientation/rotation matrix (3x3)
Unit cell lengths/angles (3 lengths)
Domain size
Domain shape
Domain orientation distribution
Incident photon spectrum
Arbitrary parameters 

Quadrant level:
Level 1 Detector Position
Arbitrary parameters 

Sensor array level:
Level 2 Detector Position
Arbitrary parameters 

ASIC level:
Level 3 Detector Position
Arbitrary parameters 

Shoebox:
Background tilt plane coefficients
Arbitrary parameters 

Conditions (goes directly into the forward model):
Shoebox pixel coordinates (position on detector)

Hyperparameter: Number of mosaic domains

Number of domains $N$ is a hyperparameter, should it be optimized?

Ways to include results from DIALS:
warm start
residual optimization
penalize deviation from DIALS

%\subsection{P-VAE for Structure Factor Amplitude Refinement}
%
%Alternative to nanoBragg
%
%Step 1: Process data in dials (including detector metrology optimization and unit cell filtering)
%
%Step 2: TDER, scaling, merging. The package \textsc{DIALS} assumes a monochromatic source, estimating a single value of $| F_{\vv{h}} |^2$ from a dataset of still shots.
%
%Step 3: Result is structure factor amplitudes $| F_{\vv{h}} |$.
%
%Step 4: Refine the structure factor amplitudes, mosaicity parameters, orientation, unit cell, incident photon spectrum, with P-VAE with incomplete forward model.



==> scraps.tex <==
We describe the Computational Crystallography Toolbox (CCTBX) for analysis of anomalous scattering corrections in serial femtosecond crystallography. Such analysis allows spatial resolution of the oxidation state of individual atoms that can elucidate charge transfer processes. However, this analysis requires strict

We describe the potential impact of using self-supervised deep learning to correct the  scientific model and provide uncertainty quantification. 

A finite crystal, as opposed to an ideal infinite one, causes broadening of the diffraction spots
is mathematically the multiplication of the shape envelope in real space, which is a convolution with the Fourier transform of the envelope in Fourier space, leading to a broadening of the diffraction spots. 


Small crystals (~10 microns per side) are imaged with serial femtosecond crystallography. In each snapshot, the crystal(s) in the frame are destroyed after a single exposure. 

One application of CCTBX is to analyze the data from serial femtosecond crystallography with x-ray free electron laser pulses. 

Talk about how there are multiple sensors, and each diffraction spot is identified by a shoebox with dials processing



Within each ASIC we draw shoeboxes


We note is is also possible for multiple crystals to be imaged in a single still shot [REF].

Each spot is integrated
Diffraction Integration for Advanced Light Sources (DIALS) is a 
DIALS estimates the orientation of the crystal by looking at the unit cell 
Diffraction spots are identified through processing by DIALS. 
Include references on how to use DIALS

Documentation of DIALS:
\url{https://dials.github.io}

Code for DIALS:
\url{https://github.com/dials/dials}

Doing nanoBragg from the start would be computationally prohibitive and starting conditions may not converge
Directly computing through the forward model
 the inverse problem would be computationally prohibitive. 
 
 
Include references on how to use nanoBragg

Integrated vs. Pixel-Level Analysis
What are the differences in analysis

DIALS completes analysis by integrating diffraction spot intensity. While integration reduces the computational burden, pixel-level information is lost. Further processing with nanoBragg refines the values derived in DIALS by attempting the pixel-by-pixel image of the spot with a simulated version.

These shifts can be extracted from SFX data;

The oxidation state of individual metal atoms in a metalloprotein can be determined by looking at the absorption edge of X-ray spectra. In particular, serial femtosecond crystallography with X-ray free electron laser pulses can allow for spatially resolving oxidation states by the determination of anomalous structure factors from diffraction data. This procedure is called spatially resolved anomalous dispersion (SPREAD).

The change in the anomalous structure factor due to the electronic environment is small, and thus there are strict requirements on the accuracy of the forward physics model. Imperfect modeling may obscure measurement of the electronic environment. 

\section{P-VAE with Forward Model Correction for Anomalous Structure Factor Determination}

Potential impact of combining deep learning with the model


How would we validate these ideas in simulation? Try a domain shape that varies, is not the same for all domains

Here, we aim to determine the source in the case of partial knowledge of a forward physics model. We assume that we have a dataset of unknown sources, with known measurements on each of the sources. We aim to undertake a joint optimization of the source parameters for each measurement, together with the parameters of a complete forward model. The objective of this optimization is to maximize the total likelihood of all measurements, with a penalty for deviating too far from the known forward physics. 

the software corrects the intensities integrated over each shoebox, and does not take into account the pixel-by-pixel variations in the shoebox. Additionally, Careless assumes zero knowledge of the underlying physics. 

The posterior distribution of the  
 account for inaccuracies in the forward model. Dalton (2022) considers integrated spots only (i.e. the only value considered is the sum of all the pixel intensities in the shoebox, not the individual pixel intensities). Each observed spot (also known as a reflection) has intensity I. This observed reflection merged intensity I is assumed to be the product of two terms: I=F, where  is the local scale factor and F is the structure factor. 

The main drawback of Careless is that the software corrects the intensities integrated over each shoebox, and does not take into account the pixel-by-pixel variations in the shoebox. Additionally, Careless assumes zero knowledge of the underlying physics. This may lead to suboptimal results as we do have knowledge of the forward model physics, even if our knowledge is incomplete.

Dalton paper for structure factors
Reference to the Dalton work here, on improving the scale factor by improving the forward model with a neural network
Note the assumptions of a prior distribution (see Design Doc for the SPREAD framework for more notes)

We assume that the non-wavelength dependent structure factors of photosystem II are known and refined by DIALS processing in prior steps; we only aim to determine the anomalous structure factor corrections. In particular, this document concerns modification of Step 11 in the current SPREAD processing pipeline. We also assume that we can measure the incident spectrum accurately (other than an unknown overall scale factor for the total flux). 

An incomplete forward model, integrated into the physics-informed variational autoencoder is considered in Yıldız (2019) and Linial (2021), in the context of ordinary differential equations (ODEs) and in Takeishi (2021) for a more general forward model. Yıldız (2019), Linial (2021), and Takeishi (2021) focus on model completion; these works do not assume sparse measurements on sources as in Mendoza (2022) and Olsen (2022).

In Yıldız (2019) and Linial (2021), sequences of a variable x in time are observed, each variable a stochastic transformation g of a latent variable z governed by an ordinary differential equation (ODE); in Linial (2021) each example is governed by an ODE of the same form but with different parameters, in Yıldız (2019) the ODE parameters are the same (unknown) values for every example. The transformation function g is unknown. A variational autoencoder takes the observed variable x as input to the encoder to find the latent space zt=0, and in the case of Linial (2021), the encoder also finds , where  are the parameters of the ODE. The decoder takes the sampled latent space variables zt=0 and , solving for the sequence of z with the underlying ODE, and converts back to a distribution over each xt with a g parameterized as a neural network.

The approaches of Yıldız (2019) and Linial (2021) are generalized with Takeishi (2021). Both the incomplete known forward model and the complete unknown forward model can take arbitrary forms in Takeishi (2021). For example, an additive or composite function parameterized by a neural network could be trained to transform the incomplete model into the completed one. The augmented forward model is penalized for veering from the known incomplete forward model through additional loss terms added to the conventional VAE loss. Takeishi (2021) and Dalton (2022) face a similar challenge: the neural network correction to the forward model can fully bypass the known physics and provide the full explanation for the measurements. Takeishi (2021) solves this by penalizing deviations from known physics, Dalton (2022) solves this by carefully selecting the metadata used in the scale factor corrections.

Yıldız (2019), Linial (2021), and Takeishi (2021) focus on model completion; these works do not assume sparse measurements on sources as in Mendoza (2022) and Olsen (2022).

In Yıldız (2019) and Linial (2021), sequences of a variable $x$ in time are observed, each variable a stochastic transformation $g$ of a latent variable z governed by an ordinary differential equation (ODE); in Linial (2021) each example is governed by an ODE of the same form but with different parameters, in Yıldız (2019) the ODE parameters are the same (unknown) values for every example. The transformation function g is unknown. A variational autoencoder takes the observed variable x as input to the encoder to find the latent space zt=0, and in the case of Linial (2021), the encoder also finds , where  are the parameters of the ODE. The decoder takes the sampled latent space variables zt=0 and , solving for the sequence of z with the underlying ODE, and converts back to a distribution over each xt with a g parameterized as a neural network.

The approaches of Yıldız (2019) and Linial (2021) are generalized with Takeishi (2021).

[Refs: Yıldız (2019) and Linial (2021)] in the context of ordinary differential equations (ODEs) and in [Ref: Takeishi (2021)] for a general forward model. 

Both the incomplete known forward model and the complete unknown forward model can take arbitrary forms in Takeishi (2021). For example, an additive or composite function parameterized by a neural network could be trained to transform the incomplete model into the completed one. 

The augmented forward model is penalized for veering from the known incomplete forward model through additional loss terms added to the conventional VAE loss. 

Takeishi (2021) and Dalton (2022) face a similar challenge: the neural network correction to the forward model can fully bypass the known physics and provide the full explanation for the measurements. Takeishi (2021) solves this by penalizing deviations from known physics, Dalton (2022) solves this by carefully selecting the metadata used in the scale factor corrections.

Recent work in Mendoza (2022) and Olsen (2022) has evaluated the use of physics-informed variational autoencoders (P-VAEs) to solve inverse problems. Specifically, these works aim to solve for the sources of a dataset of measurements. Due to physical experimental limitations, the measurement on each source is sparse. There is not enough information in the measurement to recover the source using conventional optimization methods for inverse problems. However, the entire dataset of measurements is large, i.e. there are sparse measurements on many sources. The P-VAE jointly solves for the underlying prior distribution on the sources P(source) and all the posterior distributions on the dataset, P(source | measurement).

Mendoza (2022) and Olsen (2022) use the P-VAE for computed tomography and Fourier ptychographic microscopy, respectively. Sparse measurements are assumed to be over a dataset of similar sources. In solving for the anomalous structure factors in serial femtosecond crystallography, we face a similar problem with some important differences. We have many images of crystals, and each crystal is of the same underlying material and structure factors, but has differences in the size, mosaicity, orientation, and unit cell. Our objective is to reconstruct the anomalous structure factors, which are common to all examples of the dataset. Like Mendoza (2022) and Olsen (2022), we reconstruct all the sources (i.e. crystals) of the dataset (in this case, per-source parameters such as the unit cell and orientation), but unlike in the previous work, this serves only in the larger mission to reconstruct the anomalous structure factors.

We propose a general framework for posterior estimation that is inspired by the mathematics of the variational autoencoder \cite{kingma2014autoencoding, doersch2021tutorial}. 

Deep neural networks are chosen for function approximation due to their theoretical ability to approximate any function \cite{cybenko_approximation_1989, hornik_approximation_1991, leshno_multilayer_1993} and practical success in approximating high-dimensional functions \cite{lecun_deep_2015}. 

we aim to generate diffraction spot shoeboxes $S$ from the same underlying distribution as the experimentally measured shoeboxes. 


In the proposed work, we aim to find the posterior probability distribution $P(S|M)$, where $S$ is the source being reconstructed and $M$ is the measurement.


Mendoza (2022) and Olsen (2022) use the P-VAE for computed tomography and Fourier ptychographic microscopy, respectively. Sparse measurements are assumed to be over a dataset of similar sources. In solving for the anomalous structure factors in serial femtosecond crystallography, we face a similar problem with some important differences. We have many images of crystals, and each crystal is of the same underlying material and structure factors, but has differences in the size, mosaicity, orientation, and unit cell. Our objective is to reconstruct the anomalous structure factors, which are common to all examples of the dataset. Like Mendoza (2022) and Olsen (2022), we reconstruct all the sources (i.e. crystals) of the dataset (in this case, per-source parameters such as the unit cell and orientation), but unlike in the previous work, this serves only in the larger mission to reconstruct the anomalous structure factors.


We aim to create the underlying model that generates shoeboxes that are indistinguishable from our experimentally measured shoeboxes
Minimize divergence from the modeled distribution


The proposed framework is inspired by variational autoencoders. The basic idea is to optimize the neural network such that it outputs generated shoeboxes that come from the same underlying distribution as the actual shoeboxes. More precisely, we train this structure so that the actual shoeboxes are generated with high probability (maximize P(actual shoeboxes)).

We note that the final diffraction image is  [Sauter 2020, Mendez 2020]
semantic representation
Discussion about sampling multiple mosaic domains

Each mosaic domain has a different unit cell [REF: Hattne (2014)]
need to produce a unit cell distribution for each crystal

We focus our discussion here on the anomalous corrections as a function of wavelength, though similar approaches can be utilized for finding the approximately non-wavelength dependent structure factors (when far from the \textit{K} absorption edge) as a function of Miller index

Determination of structure factor magnitude is a major step is solving the structure of macromolecules. Serial femtosecond crystallography allows for room-temperature determination of structure factors.

We present the potential impact of utilizing self-supervised physics-informed deep learning methods, and open questions for applying these techniques.

for every spot, need scale factor to account for partiality
Detector coordinates of the pixels in the shoebox are directly given in the forward model

In contrast to a conventional variational autoencoder, we do \textit{not} attempt to use this formulation to synthesize arbitrary sources $S$ by sampling $P(z)$ directly. This framework only attempts reconstruction on the training examples themselves. After training, $P(S|M)$ for every source can be sampled by first sampling $Q(z|M)$ then $P(S|z)$ (see Fig.~3). Crucially, unlike most data-driven approaches to reconstruction in computational imaging, the proposed framework assumes that no ground truth dataset of sources $S$ is available.

For efficient optimization, the variational autoencoder includes an “encoder” (with the above serving as the “decoder”). Generally, the encoder is another neural network. Here, we directly optimize the latent variables by finding a mean and variance for each latent variable, per shoebox. 

In the P-VAE, the likelihood of the data is maximized, and the 

% We aim to maximize $\log P(M) = \sum_i \log \left[ \int \int P*(M_i | S_i) P(S_i | z) P(z) dS_i dz \right]$

This is the same formulation used for the P-VAE [REF: Olsen and Mendoza]. 


We formulate as an autoencoder; the variables conditioned on are the input photon spectrum and the pixel coordinates of the shoebox (both are assumed to be known exactly).

The quantities for each level of the hierarchy are enumerated below. The distribution Q(x), where x is the latent space variable and Q is the approximation to the prior distribution, will be specified as a Gaussian with a mean and variance. There will be a latent space variable for each quantity of interest in the forward model. The mean and variance for each latent space variable will be consistent across the hierarchical level (e.g. the same for all shoeboxes in an image). The shoeboxes, as in the state-of-the-art, will be extracted using DIALS. 

The forward model may have inaccuracies that we don’t know about. Thus, at all levels (global, image, shoebox), we can optimize a set of latent variables to represent the related unknown quantities (the same as in the above image under “For each quantity.” After the “Forward Model” (bottom of the above image),  we can insert a neural network which takes in these quantities and completes further processing before outputting the predicted shoebox distribution (see below). The figure of merit to optimize the variational autoencoder will include 3 metrics: the KL divergence of the approximation with the latent variable priors, the likelihood of the data, and the KL divergence between the unmodified forward model result and the modified forward model result.

Optimizing Eqn. XX to maximize the probability of generating the experimentally measured shoeboxes is computationally difficult as given a shoebox, as most random samples will give a probability of 0 to the shoebox. We solve this problem by modifying the shoebox generator into a physics-informed variational autoencoder (P-VAE)



Processing by the \textsc{DIALS} software package yields diffraction spot shoeboxes cut from the still shot images. The shoeboxes can be represented hierarchically, with 

Figure, pg. 17

In our case, we only have a dataset of noisy measurements $M$ and no ground truth sources $O$. However, the forward model, $P(M|O)$, is known through the physics of image formation. Thus, instead of maximizing the probability of generating $O$, we can maximize the probability of generating $M$, a formulation we call the ``physics-informed variational autoencoder'' \cite{hu_physics_2022}.

Physics-informed variational autoencoder

Each shoebox is derived from an ASIC, which forms a sensor array, etc.

Talk about the generation of probability distributions as opposed to point estimates

We propose an outline for supplementing existing analysis of SFX data with physics-informed deep learning methods. Applying deep neural networks for model correction departs from existing approaches [REFs] where the forward model is carefully parameterized from first principles. The balancing of traditional processing with \textsc{DIALS} and \textsc{nanoBragg} is an open question. For example, using the shoeboxes derived from \textsc{DIALS}
For example, the results derived from \textsc{DIALS}

Number of domains $N$ is a hyperparameter, should it be optimized?

Warm start might be similar to some of the other loss functions in the Takeishi paper

The shape parameters could be a multidimensional gaussian with correlation matrix: https://doi.org/10.1107/S2053273323000682

Warm start with dials result/nanoBragg result

Hyperparameter: How many mosaic blocks to sample

Replace some of the neural networks (especially the final one) with a normalizing flow 

How should we incorporate the results from DIALS?
diffBragg - open area to switch to an automatic differentiation platform
How should we incorporate the results from DIALS/nanoBragg/diffBragg

We outline open questions and possible solutions rooted in deep learning techniques:
How many domains to model?
How to correct imperfections in forward model parametrization?

Relative detector position for each of the levels is needed

Open question: How many mosaic domains to sample?
How to make the number of mosaic domains differentiable with gradient descent?
Check transformers:
Autoregressive decoder
Stops decoding when it generates a certain token?
Keep sampling until an end condition is met.

Open question: should the unit cell and orientation and/or other parameters be independent distributions?


Allow fractional size mosaic domain, that is essentially given a smaller scale factor
a mosaic domain --> I don't think this is differentiable

Open question: How many mosaic domains to model per crystal?
Potential solutions:
Have a fixed number of domains
Or, keep sampling until stopping condition is met, the stopping condition is given by a neural network exceeding a threshold value, the threshold value could be a latent variable that is Level 1 dependent (how to make this computational efficient? Can initially sample at a high rate, and slow down as threshold value is approached)

Spatially resolved anomalous dispersion (SPREAD) utilizes nanoBragg to determine the structure factor as a function of beam energy.

Only successfully completed in simulation (Sauter 2020)

Open question: how to parametrize the shape of a mosaic domain? Could be arbitrary closed shape
Open question: how to represent the data in Level 1, the image level?
Trading off between following the scientific model and allowing model corrections
Tractable ways to deal with infinite number of domains
How best to include the output from DIALS/nanoBragg/diffBragg

Open question: penalty for deviating from the known likelihood distribution

Trading off between following the scientific model and allowing model corrections

 In photosystem II for a incident spectrum centered at 6550 eV [CHANGE TO wavelength], these atoms would be the four manganese atoms in XXX
 
 Include the equation of the wavelength dependent correction to the equation
 
 Give a general outline

Refer to Appendix

Make everything a delta of the values from DIALS/CCTBX/etc

We can separate out the terms where the anomalous scattering factor is approximately constant over wavelength, yielding:

\begin{equation}
F_{\vv{h}}(\lambda) = F_{\vv{h}, \text{ non-}{\lambda}} + \sum_{m} F_{m}(\lambda),
\end{equation}

where the summation only loops over the atoms $m$ with $K$ edge near the incident spectrum center. In photosystem II, with an incident spectrum centered at 6550 eV, the summation would concern four manganese atoms. 

our goal is primarily to find anomalous scattering factors of certain atoms; refining the structure derived from other methods is a secondary goal. For this task, our framework

Step 1: Process data in dials to draw shoeboxes, and obtain estimates of unit cell, orientation, and scale
Step 2: Process with P-VAE


Step 2: Calculate complex structure factors $F_{\vv{h}}$ without anomalous contributions using the PDB file using forward simulation code

\subsection{Open Questions}

INCLUDE IN PREVIOUS SECTION

We describe the corresponding procedure with an unknown structure in Appendix XX. 


\paragraph{How do we best incorporate the results from \textsc{DIALS} and \textsc{nanoBragg}?} 
Warm start
We don't know the ground truth source, but we do have the result from Dials/nanoBragg to warm start the encoder and decoder networks. Then we just have to refine the parameters and train the model correction network

\paragraph{How do we trade off between following the scientific model generated by first principles and allowing model corrections with deep neural networks?}
Penalize the distance between $P(M_i | S_i)$ and $P^{*}(M_i | S_i)$

\paragraph{How sensitive is the procedure to neural network architecture?}
simulated model deviations

\paragraph{How to parametrize the shape of a mosaic domain?}
Open question: how to parametrize the shape of a mosaic domain? Could be arbitrary closed shape

\paragraph{Open question: how to represent the data in the different levels?}
Metadata about the image

\paragraph{How do we verify correctness?}
Run with simulated data
Try with and without model correction
Split the data in half and try for each half (CC1/2)

More questions:

Can we remove the quality control on the unit cell? No unit cell rejection
Can we reject less data with this procedure?

Robust learned filtering

The position of each pixel relative to the crystal is described hierarchically, with Level 0 describing the overall center position, Level 1 referring to the 4 quadrants of the detector, Level 2 the 32 sensor arrays, and Level 3 the 256 application-specific integrated circuits (ASICs) [REF: Brewster 2018]. 

\section{Appendix A}

Appendix~\ref{appendix_derivation}


\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}





Hierarchical data and example images of data (unimodal worker has a way to step through data)

Encoder Input Quantities for every shoebox:

Dataset level:
N/A

Full detector image:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Overall scale factor
Measured spectrum
Orientation from DIALS
Mosaicity parameters (shape of domains, size of domains)
Unit Cell
Optimizable input variable


Quadrant level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


Sensor array level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


ASIC level:
Detector position from \textsc{DIALS} and \textsc{nanoBragg} refinement
Optimizable input variable


Shoebox:
Shoebox pixels
Background mask from DIALS
Foreground mask from DIALS
Background tilt plane coefficients from \textsc{nanoBragg}
Pixel positions
Optimizable input variable

Decoder Output Quantities:

calculated from pixel and detector positions --> Miller index from \textsc{DIALS}

Dataset level:
Anomalous corrections to scattering factors of metal atoms near the \textit{K} edge as a function of wavelength, delta from Henke tables value
atom positions in the unit cell of the metal atoms near the K-edge --> delta from known values
$B_m$ --> fixed
non-anomalous structure factor of the atom --> delta from the merging final values/nanoBragg refinement
Arbitrary parameters 
 
Full detector image:
Total flux of incident photon spectrum
Base detector position
Crystal orientation/rotation matrix (3x3)
Unit cell lengths/angles (3 lengths)
Domain size
Domain shape
Domain orientation distribution
Incident photon spectrum
Arbitrary parameters 

Quadrant level:
Level 1 Detector Position
Arbitrary parameters 

Sensor array level:
Level 2 Detector Position
Arbitrary parameters 

ASIC level:
Level 3 Detector Position
Arbitrary parameters 

Shoebox:
Background tilt plane coefficients
Arbitrary parameters 

Conditions (goes directly into the forward model):
Shoebox pixel coordinates (position on detector)

Hyperparameter: Number of mosaic domains

We can assume the structure (i.e. atom positions) is known, though the structure may be refined by adding a latent space representation and decoder for the atom positions. 

We present a general outline to perform model correction in \textsc{cctbx} for SPREAD, with the aim of generating dialog between crystallographers and machine learning researchers. 

We can minimize a loss of the following form, assuming a batch size of $n$ and a single sample:

\begin{equation}
\begin{aligned}


\text{loss} = {} & \sum_{i=1}^m \log P(M_i) = \sum_{i=1}^m \log \left[  \int \int P(M_i | S) P(S | z) P(z) dS dz \right] 
		      & \sum_{i=1}^m \log P(M_i) = \sum_{i=1}^m \log \left[  \int \int P(M_i | S) P(S | z) P(z) dS dz \right] 
\end{aligned}
\end{equation}

FIGURE: Shoebox generator (include correction network that takes as input the model correction parameters and sampled measurement), also include the hierarchical encoder in a different color

Hierarchical data encoding

A measurement $M_i$ is a diffraction spot shoebox cut from the still shot image with \textsc{dials}. The information in a shoebox can be organized hierarchically, with a shared input representation among shoeboxes cut from the same image.

Direct encoding with the dials-derived values

We describe how a similar framework can be used to refine structure factor amplitudes in Appendix~\ref{appendix_structure}.

STOPPED HERE

Alternative to nanoBragg

Step 1: Process data in dials (including detector metrology optimization and unit cell filtering)

Step 2: TDER, scaling, merging. The package \textsc{dials} assumes a monochromatic source, estimating a single value of $| F_{\vv{h}} |^2$ from a dataset of still shots.

Step 3: Result is structure factor amplitudes $| F_{\vv{h}} |$.

Step 4: Refine the structure factor amplitudes, mosaicity parameters, orientation, unit cell, incident photon spectrum, with P-VAE with incomplete forward model.


